A Supervisory Volt/VAR Control Scheme for Coordinating Voltage Regulators with Smart Inverters on a Distribution System

This paper focuses on the effective use of smart inverters for Volt/Var control (VVC) on a distribution system. New smart inverters offer Var support capability but for their effective use they need to be coordinated with existing Volt/Var schemes. A new VVC scheme is proposed to facilitate such coordination. The proposed scheme decomposes the problem into two levels. The first level uses Load Tap Changer (LTC) and Voltage Regulators (VRs) and coordinates their control with smart inverters to adjust the voltage level on the circuit to keep the voltages along the circuit within the desired range. The second level determines Var support needed from smart inverters to minimize the overall power loss in the circuit. The results of the supervisory control are sent to the devices which have their local controllers. To avoid frequent dispatch, smart inverters are supervised by shifting their Volt/Var characteristics as needed. This allows for the smart inverters to operate close to their optimal control while meeting the limited communication requirements on a distribution system. A case study using the IEEE 34 bus system shows the effectiveness of this supervisory control scheme compared to traditional volt/var schemes.

==> _figures/4_VRLTCModule <==
<?xml version="1.0" encoding="UTF-8" standalone="no"?>
<!-- Created with Inkscape (http://www.inkscape.org/) -->

<svg
   width="297mm"
   height="210mm"
   viewBox="0 0 297 210"
   version="1.1"
   id="svg5"
   inkscape:version="1.2.1 (2ed6d7ae0b, 2022-08-22, custom)"
   sodipodi:docname="4_VRLTCModule"
   xmlns:inkscape="http://www.inkscape.org/namespaces/inkscape"
   xmlns:sodipodi="http://sodipodi.sourceforge.net/DTD/sodipodi-0.dtd"
   xmlns="http://www.w3.org/2000/svg"
   xmlns:svg="http://www.w3.org/2000/svg">
  <sodipodi:namedview
     id="namedview7"
     pagecolor="#ffffff"
     bordercolor="#666666"
     borderopacity="1.0"
     inkscape:showpageshadow="2"
     inkscape:pageopacity="0.0"
     inkscape:pagecheckerboard="0"
     inkscape:deskcolor="#d1d1d1"
     inkscape:document-units="mm"
     showgrid="true"
     inkscape:zoom="1.829812"
     inkscape:cx="851.18034"
     inkscape:cy="425.72679"
     inkscape:window-width="3806"
     inkscape:window-height="2126"
     inkscape:window-x="14"
     inkscape:window-y="14"
     inkscape:window-maximized="1"
     inkscape:current-layer="layer1">
    <inkscape:grid
       type="xygrid"
       id="grid132"
       originx="0"
       originy="0" />
  </sodipodi:namedview>
  <defs
     id="defs2" />
  <g
     inkscape:label="Layer 1"
     inkscape:groupmode="layer"
     id="layer1">
    <ellipse
       style="fill:none;stroke:#000000;stroke-width:0.731472;stroke-dasharray:none"
       id="path236"
       cx="139.66223"
       cy="22.625311"
       rx="20.702515"
       ry="5.0206213" />
    <text
       xml:space="preserve"
       style="font-style:normal;font-weight:normal;font-size:5.64444px;line-height:1.25;font-family:sans-serif;fill:#000000;fill-opacity:1;stroke:none;stroke-width:0.264583"
       x="123.93056"
       y="24.397467"
       id="text1058"><tspan
         sodipodi:role="line"
         id="tspan1056"
         style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size:5.64444px;font-family:sans-serif;-inkscape-font-specification:'sans-serif, Normal';font-variant-ligatures:normal;font-variant-caps:normal;font-variant-numeric:normal;font-variant-east-asian:normal;stroke-width:0.264583"
         x="123.93056"
         y="24.397467">Start (k=0)</tspan></text>
    <rect
       style="fill:none;stroke:#000000;stroke-width:0.499999;stroke-dasharray:none"
       id="rect1162"
       width="84.672745"
       height="25.208414"
       x="60.931942"
       y="46.592766"
       ry="6.614583" />
    <text
       xml:space="preserve"
       style="font-style:normal;font-weight:normal;font-size:10.5833px;line-height:1.25;font-family:sans-serif;fill:#000000;fill-opacity:1;stroke:none;stroke-width:0.264583"
       x="39.524227"
       y="114.04847"
       id="text1166"><tspan
         sodipodi:role="line"
         id="tspan1164"
         style="stroke-width:0.264583"
         x="39.524227"
         y="114.04847">$Tap_{LTC}(k) = Tap_{LTC}^0 + \Delta Tap_{LTC}^p$</tspan></text>
  </g>
</svg>

